TorontoCity: Seeing the World with a Million Eyes

In this paper we introduce the TorontoCity benchmark, which covers the full greater Toronto area (GTA) with 712.5 $km^2$ of land, 8439 $km$ of road and around 400,000 buildings. Our benchmark provides different perspectives of the world captured from airplanes, drones and cars driving around the city. Manually labeling such a large scale dataset is infeasible. Instead, we propose to utilize different sources of high-precision maps to create our ground truth. Towards this goal, we develop algorithms that allow us to align all data sources with the maps while requiring minimal human supervision. We have designed a wide variety of tasks including building height estimation (reconstruction), road centerline and curb extraction, building instance segmentation, building contour extraction (reorganization), semantic labeling and scene type classification (recognition). Our pilot study shows that most of these tasks are still difficult for modern convolutional neural networks.

==> aerialImages.tex <==

\gellert{
We use aerial images provided by City of Toronto covering the whole Greater Toronto Area (GTA).
 The images were acquired in the spring 2011, they are orthorectified to $10 cm/pixel$ ground resolution, they have 4 channels (Red, Green, Blue, Near infrared) and 16 bit resolution. 
We projected each image to the Universal Transverse Mercator (UTM) 17 zone in the WGS84 geographic datum and tiled the area to $500\times500m^2$ images without overlap. 
The images have high geometric accuracy on the ground ($\approx 10 cm$), however the are not true orthophotos and thus high buildings can cause misalignments. 
}
 

==> creatingBenchmark.tex <==
Manually labeling such a large scale dataset is not possible. 
For example, \cite{Mattyus} reported that $21h/km^2$ was necessary to label aerial images of the city of Karlsruhe with road, building, sidewalk, parking and lane markings.
Thus it will take approximately 2 years to label  one set of aerial images of TorontoCity with only those classes. 
Note that semantic segmentation is only one of the many tasks that we want to create and we have many sources of information (i.e., aerial, panoramas, LIDAR, stereo). 
Since human labeling is thus not possible, and MTurk is not precise enough, in this paper we resort to existing 2D and 3D map data to alleviate the labeling process. 
In this section we describe the map data we utilize for creating our ground truth. 
We then show how we can use this map data to easy the labeling task. 
%Labeling semantic segmentation in aerial image took Labeling aerial images takes on average XX \raquel{add some stats of what the actual price will be}. 

In this section we describe our algorithms to align automatically maps with our different sources of imagery. We then describe how to convert the road data into semantic segmentation. 

%\gellert{ The description of the objects in the world with their geospatial coordinates is the task of making maps (cartography) and it is practiced since the ancient times of humanity. 
%A map has to fulfill certain quality requirements (e.g. the accuracy and the structure of the annotations, the used coordinate system, etc.) and therefore it it performed by skilled persons (cartographers).
%On one hand this leads to higher labor costs, but on the other hand the already existing maps can be used as annotations. 
%Our estimate is that the annotation (mapping) of $1km^2$ takes at least 10 hours of work, thus the annotation of the covered area ($712.5km^2$) would take around $300$ days net labor time which would imply high costs. 
%Additionally, our dataset includes ground images (panoramas, lidar, stereo images) which adds more images to annotate.
%Getting the ground truth by manual labeling on this scale is unfeasible, therefore we take advantage of different map sources and align the different data sources so that the map (labeling) information can be transferred between them. }

%\shenlong{Not sure whether we need two levels subtitles...} 
%\subsubsection{Map sources}


%Our ground-truth is acquired from multiple forms of high-precision maps of Toronto. Compared to online map services such as  OpenStreetMap \cite{OSM} and Google Maps, the provided data is more accurate and up-to-date and  contains much more detailed meta information, such as buildings' height, building 3D shape and accurate road curbs. Most importantly, all of the maps we use are perfectly registered (i.e., aligned with each other) and are aligned with the aerial images as shown in \figref{fig:task}. 
%This allow us to create large-scale ground-truth information for benchmarking multiple computer vision tasks. 
%We now briefly introduce the map layers that we have used to construct our TorontoCity dataset. 

%\paragraph{Road Maps:}
%This   map contains  polylines representing streets, sidewalks, rivers and railways within the City of Toronto. Each line segment is described with a series of attributes such as  a unique identifier, name, road category and address range. \raquel{what is address range?} Road  intersections are explicitly encoded as intersecting points between polylines. 
%This allows us to create our road topology benchmark. % of automatic road network generation. 
%Moreover, road curbs  are also available, which we exploit for our road semantic segmentation tasks.  We refer the reader to \figref{fig:map} depicts an example of the road curb data overlayed with aerial images. \raquel{It is not clear what we want to show here.}

%\paragraph{Property Maps:}
%This  map contains  the location and footprint of buildings as well as several attributes for those buildings such as their  addresses,  height and  elevation. 
%We utilize this map for semantic and instance labeling as well as building height estimation. This map was created  by the City's department of urban planning and design, and the accuracy of geometry surpasses most human annotators in terms of polygon representation, as shown in \figref{fig:map}. \raquel{do we have evidence of this? do we know how this map was created?}
% The Property Data Maps (PDM) provided by the city of Toronto defines precisely the curb (edge) of the road.

%\paragraph{Urban Zoning Maps:}
%This map  describes the government control  of the use of land, and of the buildings thereon. The government divides  land into zones, within which various uses are permitted but not others. For instance, for the city of Toronto, the main categories of urban zoning includes residential, commercial, industrial, institutional, \etc. Note that for one zone multiple purposes are allowed, such as commercial+residential. This allows us to create a multi-class pixel-wise  labeling tasks in both bird's eye and ground views.  Solving this visual task is important for urban planning, real estate and law-enforcement. \raquel{pass this sentence to where we describe the tasks} %We believe that there is enough visual evidence for humans to tell the functioning of the region. Whether computers are able to learn such high-level information from labeled data is both intriguing and of pratical use. 

%\paragraph{3D  Maps:}
%This map  contains  3D shapes for all the $400,000$ buildings in the GTA area. 
%The level of detail varies per building. For many buildings, as shown in \figref{fig:3d}, the level of precision is cm accurate and contains many other semantic primitives such as windows and balconies. We plan to use such building for our facade parsing and normal estimation benchmark, and all buildings for the building height estimation task. 
%\raquel{We haven't yet talk about normal estimation in the subsection before about tasks to come}
%This provides centimeter level accurate geometry in 3D. For a subset of buildings it also contains information such as assets on facades, such as windows and balconies, as shown in \figref{fig:3d}. 
%This would potentially bring an accurate ground-truth multiple tasks from ground-view, such as facade parsing, ground-view building segmentation, instance segmentation, normal estimation and depth estimation. 
%\shenlong{todo in supp: more figures for maps and more stats\\
%maybe put stats here?}
% Shenlong or Hang could you explain this here? }

%\section{Generating Ground Truth from Maps}

\subsection{Map Sources}

\paragraph{Road Maps:} {\color{red}{What did you use?}}

\paragraph{Property Maps:} This  map contains  the location and footprint of buildings as well as several attributes for those buildings such as their  addresses,  height and  elevation. 
%We utilize this map for semantic and instance labeling as well as building height estimation. This map was created  by the City's department of urban planning and design, and the accuracy of geometry surpasses most human annotators in terms of polygon representation, as shown in \figref{fig:map}.

\paragraph{Urban Zoning Maps:} {\color{red}{What did you use?}}

\paragraph{3D  Maps:} {\color{red}{What did you use?}}


%\paragraph{Building footprints:}
%For the aerial images the footprints can be applied directly. 

\subsection{Aligning maps with ground images}

\raquel{say that you do it via the aerial images as maps are sparse data}

It is worth noting that the streetview panoramas have noticable noise (usually between 1-3 meters) in geolocation. This noise results in a misalignment with both the aerial images and the 3D maps, which hurts the quality of applying the 3D maps directly over the streetview panoramas. However, given the fact that the aerial images are aligned almost perfectly with the map. We proposed a simple yet effective aerial-ground view alignment based on rectified streeview panoramas. To be specific, we first rectify the panoramas by projecting pixels from 360 sphere onto the ground-plane. We extract the image of the ground-plane region between $[-20, 20]\times[-20, 20]$ meters with $10$cm/pixel and get a $400\times400$ rectified image, as shown in \figref{fig:ncc}. After that the alignment is conducted between the rectified ground-view and aerial images. We then maximize the following function wrt the camera's offsets along three dimensions:
\[
(x, y, z) = \arg \max f_\mathrm{NCC} (I^\mathrm{aerial}_{x, y}, I^\mathrm{ground}_z) + \lambda f_\mathrm{Prior}(x, y, z)
\]
where $(x, y, z)$ is the camera's offsets; $I^\mathrm{aerial}_{x, y, z}$ is a patch of the $I^\mathrm{aerial}$ with the centroid to by $(x_0+x, y_0+y)$; $I^\mathrm{ground}_z$ is the re-scaled ground-view images according to the camera height $z$. $ f_\mathrm{NCC}$ is the NCC score between the ground image and a patch of the aerial image with a given offset $(x, y, z)$: 
\[
f_\mathrm{NCC}(I^1, I^2) = \frac{1}{n} \sum_{u, v} \frac{(I^1(u, v) - \bar{I}^1)(I^2(u, v) - \bar{I}^2)}{\sigma_{I^1} \sigma_{I^2}}
\]
And $f_\mathrm{Prior}$ is a Gaussian prior over the offsets:
\[
f_\mathrm{Prior} = \exp\left(- \left(\frac{x^2}{\sigma_{x}^2} +\frac{y^2}{\sigma_{y}^2}+ \frac{(z - 2.5)^2}{\sigma_z^2}\right)\right)
\]
In practice we choose $\sigma_x = \sigma_y = 2$ and $\sigma_z = 0.2$. The intensity range of both aerial and ground images rescaled to $[0, 1]$ before NCC computing and our balancing parameters $\lambda$ is chosen to be $0.3$. The solution space is a discrete search window in the range $[-10, 10]\times[-10, 10]\times[2.2, 2.6]$ with a step of $0.1$. Thus the cardinality of the search space is $201\times 201\times 5$. The search is conducted in an exhaustive search manner. Note that the NCC score map can be conducted efficiently through fast FFT trick, with a $M^2 log_2 M$ complexity. And the gaussian prior score is a fixed LUT. Fig.~\ref{fig:ncc} depicts the image overlay before and after our alignment, as well as the camera locations before/after the alignment. \shenlong{The NCC based alignment on the top-down view gives us good coarse localization of the camera but does not necessarily brings per-pixel label accuracy when projecting the map onto the panoramas. This is mainly due to the constraint of the resolution from the top-down. In order to achieve more accurate label, we have an additional fine localization based on the consistentcy between projected road curb on the ground-view and the curb detection from the panorama. To be specific, given a camera pose hypothesis, we project the road curb polylines onto the panorama and count the number of inliers in terms of whether the projected road curb map are within 3 pixels of an image boundary detected from the panorama. We adopt the structured edge is the boundary detector here. We search over an $[-1m, 1m]\times [-1m, 1m]$ region with a step of 5cm to achieve better aligned results. }
However, this top-down view alignment is not perfect due to the clutters present in ground-view images, non-flat terrain, \etc. This would results in the quality of the ground-truth per-pixel labels in the streetview images. In order to provide ground-truth annotations with subpixel level accuracy, we conduct a fast manual pass over all the images and discard those streetview images with imperfect ground-truth. This is the only manual annotation in the whole dataset and it takes less than {\color{red} xx} sec per each panorama. Finally it gives us {\color{red}xx} images per $0.25km^2$. Please refer to the supplementary materials for more detailed information about the alignment. 

\shenlong{todo in supp: sphere to ground projection equation. Detailed equation on how to extract the aerial patch; }
\paragraph{•}

We take advatange of high-resolution cadastral maps to create labeled ground-view. To be specific, we exploit 3D building map and the property map and project the them onto the panoramas given our estimated geolocation of the panoramas. To be specific we create the large-scale road segmentation and zoning-type image classification ground-truth. The whole manual filtering only takes xx minutes to generate xx images with pixel-wise ground-truth annotation adn takes no time for the image level scene type. \figref{fig:seg} show the result of final pixel-level annotations on our dataset.

% Furthermore, labeling XX panoramas. Instead we take advantage of high resolution cadastral maps, XX and YY. Towards this goal, we need to align the maps with the aerial images as well as the panoramas. 
 
 
  \begin{figure*}[t]
 \includegraphics[width=0.99\linewidth]{fig/task/source.png}
 \caption{Examples of data collected}
 \label{fig:data}
 \end{figure*}
 
   \begin{figure*}[t]
   \centering
 \includegraphics[width=0.99\linewidth]{fig/task/map.png}
 \caption{Examples of maps}
 \label{fig:map}
 \end{figure*}
 
% \raquel{Talk about how this is done} Shenlong describe your stuff
 
 %\raquel{Gellert not sure if we need to describe the creating of the semantic segmentation. }
 
 \subsection{Semantic Segmentation from Polyline data}
 
 \raquel{Talk first about what the problem is, and illustrated with a figure. Then show how to did an automatic method to obtain  the segmentations. Give details about this }
 \gellert{
The available maps provide two types of polyline structures about roads: curbs (edges of roads) and road center lines which also define the connectivity (adjacency) in the street network. 
To generate the road surface we assign the curbs to road center lines and generate polygons based on this. 
Unfortunately, the two input data are not perfectly aligned and there is no obvious one to one match, therefore we have to reason about the assignment by including priors about the connectivity. 
Figure \ref{fig:roadSurfaceGeneration} shows an example for the road surface generation.

To solve the assignment problem we define an MRF with unary and pairwise term reasoning about the assignment of each curb segment $y_i$ to a road center line. The states of $y_i$ are the $k$ nearest road line segments $r_k$ around the $i$th curb segment plus a state for no match, $y_i=[0,1,\dots,K]$. 
We define the unary terms $\phi_{un}(y_i)$ based on the distance of $y_i$ to $r_k$ and the heading difference between $y_i$ and $r_k$. The pairwise term $\phi_{con}(y_i,y_{i+1})$ expresses that two consecutive curb segments should be assigned to adjacent road center line segments: 
\begin{equation}
\phi_{con}(y_i, y_{i+1}) = 
\begin{cases}
0 &\text{if } r_{y_i} \text{ and } r_{y_{i+1}} \text{are adjacent} \\
\lambda &\text{otherwise} 
\end{cases}
\label{eq:curbConnectivityPairwise}
\end{equation}
, where $\lambda$ is a large constant enforcing the connectivity.

The curbs (road boundaries) are naturally a single loop, we approximate this by a chain where the start and endpoint is the same. 
In some cases there are branches in the curbs (noise in the input data), in this case we handle them as separate chains. The energy for a curb with $N$ segments can be described as: 
\begin{equation}
E(\mathbf{y}) = \sum_{i=1}^N \phi_{un}(y_i) + \sum_{i=1}^{N-1}\phi_{con}(y_i, y_{i+1})
\label{eq:CurbAssignmentEnergy}
\end{equation}
The assignment is the one with the lowest energy: $\mathbf{y}^* = \arg\!\min{E(\mathbf{y})}$ , which can be computed exactly by dynamic programming. 
Our formulation allows multiple curbs to be matched to one road, which is needed to form a road with curbs on both side. In some cases it occurs that there is no road for the curb or there are no curbs for a road center line, we neglect these areas and consider them as background. 
This has to be considered as labeling noise.  


  \begin{figure}[ht]
 \centering
%\begin{subfigure}[t]{0.135\textwidth}
 %\includegraphics[width=\textwidth]{fig/map/roadCurbs.png}
 
  %\end{subfigure}
\begin{subfigure}[t]{0.48\linewidth}
 \includegraphics[width=\linewidth]{fig/map/roadCurbsImage.jpg}
\caption{}
\label{fig:roadSurfaceGeneration_Input}
 \end{subfigure}
 \begin{subfigure}[t]{0.48\linewidth}
 \includegraphics[width=\linewidth]{fig/map/roadCurbsImageRoadSurface.jpg}
\caption{} 
\label{fig:roadSurfaceGeneration_Final}
 \end{subfigure}

 \caption{Example for the road surface generation. (a) shows the input data: the curbs in yellow and the center lines in red. The extracted road surface is the union of polygons (blue fill color and black edge color) generated from the assignment between the curbs and center lines. Note that a formulation ensuring connectivity is needed, otherwise the road surface would contain holes at intersections.}
 \label{fig:roadSurfaceGeneration}
 \end{figure} 
 
 }
